Comparing Self-Disclosure Themes and Semantics to a Human, a Robot, and a Disembodied Agent

As social robots and other artificial agents become more conversationally capable, it is important to understand whether the content and meaning of self-disclosure towards these agents changes depending on the agent's embodiment. In this study, we analysed conversational data from three controlled experiments in which participants self-disclosed to a human, a humanoid social robot, and a disembodied conversational agent. Using sentence embeddings and clustering, we identified themes in participants' disclosures, which were then labelled and explained by a large language model. We subsequently assessed whether these themes and the underlying semantic structure of the disclosures varied by agent embodiment. Our findings reveal strong consistency: thematic distributions did not significantly differ across embodiments, and semantic similarity analyses showed that disclosures were expressed in highly comparable ways. These results suggest that while embodiment may influence human behaviour in human-robot and human-agent interactions, people tend to maintain a consistent thematic focus and semantic structure in their disclosures, whether speaking to humans or artificial interlocutors.

==> tex/data_collection.tex <==
\section{Data Collection}


==> tex/tables.tex <==
\begin{table*}[ht!]
\centering
\caption{LLM generated Labels and Descriptions after clustering responses for experiments 1,2, and 3}
\label{tab:clusters}
\scalebox{0.9}{
\begin{tabular}{|c|p{1.7cm}|p{16cm}|}
\hline
\textbf{Exp.} & \textbf{Cluster Label}
& \textbf{Description}                                                                                             \\ \hline

\multirow{3}{*}{\textbf{1}}
& \textbf{Financial Independence and Adjustment in Academic Pursuits}
& This cluster highlights the transition from familial financial support to a greater reliance on personal finances among students pursuing higher education. A recurring theme centers on the challenges and adjustments associated with managing finances while balancing academic responsibilities. Some students exhibit increased awareness and anxiety around budgeting and financial management due to using their own funds or navigating student loans for the first time. Responses reflect a range of experiences, from those fortunate enough to have governmental support or scholarships covering their fees to others who acknowledge the complexity and stress of financing their education independently. Many respondents initially struggle with balancing work and school but gradually adopt better strategies, indicating a learning curve that relates to both financial literacy and time management. The contrast between previous reliance on family support and present self-sufficiency emerges as a significant concern, along with the unexpected costs of living and studying abroad, which compound the pressure to maintain adequate financial stability while achieving academic goals.
\\ \cline{2-3}
& \textbf{University Life Balance and Social Integration}
& The responses in this cluster reveal a nuanced perspective on the relationship between academic responsibilities and social life during university. A recurring theme is the struggle to establish a balance between academic demands, such as coursework, readings, and feedback processes, and the desire for social engagement, particularly through extracurricular activities and casual interactions. Participants indicate that their social experiences are often intertwined with university life, suggesting that friendships are predominantly formed within academic settings. Concerns about achieving a balanced lifestyle emerge, with some respondents feeling overwhelmed by the intensity of their academic schedules, leading to reduced social time. While some have found ways to integrate social activities into their academic routines, others express a commitment to prioritize their studies, reflecting a transitional phase where social exploration is temporarily sidelined in favor of academic success. Overall, these insights highlight the complex dynamics of university life, where students navigate the pressures of academic rigor alongside a longing for social connection.
\\ \cline{2-3}
& \textbf{Insufficient Lecturer Feedback}
& The responses in this cluster reflect a prevalent concern among students regarding the lack of personalized feedback from lecturers, particularly in large lecture settings. Many students expressed frustration that they primarily receive feedback from tutors rather than directly from their lecturers, leading to a feeling of disconnection and a lack of individual recognition. The responses indicate that the size of the classes contributes significantly to this issue, as students feel that lecturers do not have the capacity to provide meaningful feedback when addressing hundreds of students at once. While students appreciate the importance of feedback for personal improvement and educational growth, they highlight a notable deficit in receiving timely and constructive critiques on their assignments. This lack of interaction is often compounded by inefficient communication practices, where lecturers may rush through answering questions or take too long to respond to emails. Overall, the cluster reveals a strong desire for more engaged and accessible feedback mechanisms from lecturers to enhance the learning experience. 
\\ \hline
 
\multirow{3}{*}{\textbf{2}}
& \textbf{Financial Awareness and Minimal Budgeting}
& This cluster reveals a pragmatic approach to financial management characterized by basic budgeting practices and a reliance on personal awareness rather than detailed tracking. Respondents typically maintain two bank accounts, one for daily expenses and another for bill payments, allowing them to compartmentalize their finances. While some individuals utilize spreadsheets to outline annual expenses and facilitate budget planning, others exhibit a more casual attitude, managing finances with a general sense of their income and expenditures. Notably, a common theme is the absence of a rigorous financial tracking system, with respondents expressing confidence in their intuitive understanding of their financial situation. Overall, the insights suggest a blend of structured habits for those who actively engage in budgeting, contrasted by a more relaxed mindset among others who feel less compelled to monitor their finances closely, often leading to a sense of security as they report sufficient funds remaining at the month’s end.
\\ \cline{2-3}
& \textbf{Family Relationships and Dynamics}
& The responses reflect a diverse yet largely positive landscape of family relationships. Many individuals express a strong sense of closeness with siblings and parents, indicating supportive and nurturing family environments. The presence of extended family contributes to a feeling of stability and connection, particularly for those who are single parents, demonstrating the importance of familial involvement in child-rearing. However, there are nuanced dynamics, such as varying relationships with parents, particularly in cases of divorce or loss, which suggest that while many feel a strong bond with their families, there are also challenges that arise from changing family structures. Communication patterns also vary, with some individuals maintaining infrequent contact yet still valuing the quality of interactions when they do meet. Overall, this cluster highlights both the strength of familial ties and the complexities that can accompany them, showcasing a blend of affection, support, and the occasional tensions inherent in family dynamics.
\\ \cline{2-3}
& \textbf{Social Engagement and Leisure Activities}
& This cluster reveals a strong focus on social interaction and personal leisure activities among a diverse group of individuals. Many responses highlight the importance of socializing, particularly on weekends, as a means to relax and unwind from the demands of work or studies. The emphasis on engaging with a core group of friends indicates a preference for maintaining close connections, which fosters a sense of community and support. Additionally, retirees express satisfaction in utilizing their spare time for various hobbies such as gardening, volunteering, and sports, showcasing the fulfillment derived from active involvement in both solitary and communal activities. A notable trend is the incorporation of physical and mental wellness pursuits, like yoga and boxing, emphasizing a holistic approach to self-care in conjunction with social life. Overall, the responses depict a balanced lifestyle that values both companionship and individual interests, signifying the participants’ efforts to nurture well-being amid their responsibilities.
\\ \hline

\multirow{3}{*}{\textbf{3}}
& \textbf{Balancing Academic Demands and Social Well-being}
& The responses reflect a strong emphasis on the importance of maintaining a balance between academic responsibilities and social interactions for mental well-being. The participants, primarily students juggling their studies and work commitments, highlight socializing with friends and family as a critical source of support and relief from stress. The integration of leisure activities, such as going to the gym, engaging in sports, reading, and pursuing creative hobbies like painting, serves as essential coping strategies to mitigate the pressures of university life. There is a notable trend of prioritizing social relationships, with participants acknowledging their dependence on these interactions to enhance their self-esteem and overall happiness. Even amidst the chaos of academic demands, there is a clear recognition of the need to actively pursue social experiences to foster resilience and maintain a sense of stability.
\\ \cline{2-3}
 & \textbf{Physical Fitness and Well-being}
 & The responses in this cluster reflect a generally positive attitude towards physical health and fitness, with most individuals indicating a commitment to regular exercise and a balanced diet. Common activities include gym workouts, walking, and participation in sports such as tennis, highlighting a preference for varied physical activities. However, there is an undercurrent of fatigue and acknowledgment of not always being at optimal fitness levels, with mentions of tiredness and "niggling injuries." While individuals strive for a healthy lifestyle, balancing academic or work commitments with exercise appears to be a significant challenge, leading to some expressing concerns about their overall health relative to their goals. The emphasis on incorporating nutrient-rich foods and aiming for specific fitness targets, like achieving 10,000 steps a day, shows an awareness of health and wellness, indicating a desire for personal improvement despite time constraints.
 \\ \cline{2-3}
 & \textbf{Balancing Social Connections}
 & The responses in this cluster reflect a nuanced perspective on social relationships and the balance between in-person interaction and virtual connections. Key themes include the value placed on close family bonds, particularly with immediate family members, and the importance of nurturing friendships both in-person and online. Many individuals express a blend of introversion and a desire for social engagement, indicating that while they enjoy spending time with friends—whether through organized meetups or casual evenings in—they also appreciate the comfort of solitude. There is a recognition of the challenges in balancing relationships across different geographical locations, with respondents expressing gratitude for their supportive social networks. The overall sentiment conveys an understanding that maintaining these connections, whether through physical presence or digital communication, contributes significantly to their well-being and happiness. This cluster illustrates different approaches to socializing, showcasing a mix of extroverted tendencies alongside a preference for quieter, more reflective social engagements.
\\ \hline

\end{tabular}}
\end{table*}
